Wireless earbuds for low-cost hearing screening

We present the first wireless earbud hardware that can perform hearing screening by detecting otoacoustic emissions. The conventional wisdom has been that detecting otoacoustic emissions, which are the faint sounds generated by the cochlea, requires sensitive and expensive acoustic hardware. Thus, medical devices for hearing screening cost thousands of dollars and are inaccessible in low and middle income countries. We show that by designing wireless earbuds using low-cost acoustic hardware and combining them with wireless sensing algorithms, we can reliably identify otoacoustic emissions and perform hearing screening. Our algorithms combine frequency modulated chirps with wideband pulses emitted from a low-cost speaker to reliably separate otoacoustic emissions from in-ear reflections and echoes. We conducted a clinical study with 50 ears across two healthcare sites. Our study shows that the low-cost earbuds detect hearing loss with 100% sensitivity and 89.7% specificity, which is comparable to the performance of a $8000 medical device. By developing low-cost and open-source wearable technology, our work may help address global health inequities in hearing screening by democratizing these medical devices.

==> intro.tex <==
\section{Introduction}
\vskip 0.15in

%It is estimated that 5.3% of the world’s population suffers from disabling hearing loss. Also, a disproportionate brunt of this problem falls on low- and middle-income countries (LMICs)1. Hearing loss can be especially harmful for neurodevelopment if untreated in early childhood. However, the impact of hearing loss may be mitigated when detected and treated early2. It is common practice for high-income countries to adopt guidelines for universal infant hearing screening using otoacoustic emission (OAE) or auditory brainstem response (ABR)3 testing. In spite of this, the test equipment remains expensive and costs thousands of dollars, which contributes to limited hearing screening in LMICs. In these countries, access to hearing assessment and equipment often requires travel to an urban setting and long wait times4,5.



The World Health Organization estimates that 5.3\% of the world's population suffers from disabling hearing loss and 80\% of people who need hearing care live in  low and middle-income countries~\cite{who_hl,mcpherson2012newborn,swanepoel2010telehealth}. Hearing loss is particularly harmful for neuro-development if it is left undetected in early childhood~\cite{standard2,standard3,nbme22}. As a result, high-income countries  have guidelines for universal infant hearing screening --- the Joint Committee on Infant Hearing, the  American Academy of Pediatrics and  the Centers for Disease Control and Prevention all recommend  universal hearing screening~\cite{standard2,standard3,standard1,standard4} that is now implemented across almost all states, communities and hospitals in the United States~\cite{patel2011universal,cdc}. 


Since the neonatal population cannot provide behavioural response to conventional audiometry tests~\cite{app3,app1,app2,walker2013audiometry}, existing newborn hearing screening technologies instead use the sounds generated by a healthy cochlea called otoacoustic emissions 
(OAE)~\cite{abdala2001distortion,chan2022inner}. While we think of the ear as a biological organ that receives sounds like a microphone, a healthy cochlea, the part of the inner ear responsible for converting sound waves into electronic impulses for the brain, also generates sounds.   These emissions  are created when the cochlea's sensory hair cells vibrate in respond to external sounds~\cite{abdala2001distortion,thompson2001universal,torre2003distortion}. So we could pick up these faint sounds and use their absence to detect hearing loss.


The challenge is that picking up these faint  sounds  from the cochlea requires sensitive acoustic hardware and medical devices  that are expensive (5000-8000 dollars)~\cite{product1,product2}. As a result,  there is limited to no-hearing screening in low and middle-income countries~\cite{india1,kenya1}.  Further, in rural and resource-limited settings, getting access to hearing assessment  may often require travel to an urban setting and  long wait times, significantly limiting the accessibility of hearing care~\cite{mcpherson2012newborn,swanepoel2010telehealth,nbme22}.

Given the importance of expanding hearing screening to low- and middle-income countries, recent work~\cite{nbme22}  uses a low-cost smartphone attachment to detect otoacoustic emissions. However, prior work  has multiple   limitations that limit its adoption in the target use-cases.
\squishlist
%This calibration is needed to ensure that recorded OAEs are above a predetermined sound level threshold. 
%Since the microphone and speaker hardware across smartphone models is different, the same digital sound output index specified in software would result in a different sound level produced at the speaker for different smartphone models~\cite{nbme22,heitmann2021mass,heitmann2017sound4all}. Similar sound level calibration also needs to be performed for the microphone to find the mapphttps://www.overleaf.com/project/636f2a2b36d9358c83b76c4aing between the recorded digital value and the corresponding absolute sound level. This calibration has to be manually performed for each new smartphone model making it hard to generalize the system. %  to multiple clinics, 

% Prior work proposes attachments that use the smartphone's  audio processing chain that particularly impacts the OAE thresholds. Specifically,
%These clinic rooms may have poor soundproofing and   doors made of corrugated metal or thin wood that do not fully close. 
%The use of a medical device that has a do-it-yourself (DIY) component presents challenges in adoption from clinicians.
%the quality of the OAE test, and more broadly

\begin{figure}[t!]
\vskip -0.15in
\centering
    % \includegraphics[width=.4\textwidth]{./figs/fig1}
    \includegraphics[width=.35\textwidth]{./figs/fig1b}
    % \includegraphics[width=.4\textwidth]{./figs/fig1c}
    \vskip -0.05in
\caption{{\bf OAEbuds in use with an infant.} Our low-cost wireless earbud can perform  hearing screening by detecting otoacoustic emissions (OAE) from the cochlea.}
\vskip -0.15in
\label{fig:fig1}
\end{figure}

\item  {\it Generalization across smartphones.}   These smartphone attachments require calibration of both the speaker and microphone sound levels to accurately detect OAEs. Since these levels vary across the different microphone and speaker hardware used in various smartphone models, these are manually calibrated for each smartphone. This  makes it hard to generalize the system to the large diversity of smartphones used across the world.
\item {\it Robustness issues with  using multiple speakers.} Prior work~\cite{nbme22} repurpose the two speakers on a wired  earphone to transmit two different tones into the ear canal. The cochlea has a non-linear response and so it  generates a third inter-modulated frequency, which can be used to reliably identify  OAEs.   Since low-cost speaker hardware have non-linearities that  also generate inter-modulated frequencies, the use of two  speakers allows prior work to develop a workaround for hardware non-linearities. These multiple speakers however are manually connected using    tubes, which is less robust. 

%\item  {\it Susceptibility to background noise.} OAE tests are highly sensitive to background noise due to their faint levels, and are  performed in quiet clinic settings~\cite{hopkins} to obtain reliable results. In low and middle income countries, neighborhood clinics  are often  next to busy roads, leading to increased levels of ambient noise. As a result, commercial OAE devices frequently produce errors due to background noise  common in these settings. % and the test often has to be conducted multiple times, which lead to patient discomfort and protracted clinic visits.
\item {\it Limited adoption for DIY devices.}  The use of tubes  and wires that are manually connected  to design a low-cost OAE probe introduces a DIY aspect to the system. In an informal survey of clinicians in Nairobi, Kenya, conducted by the authors, participants noted that the DIY-aspect of a low-cost probe could translate to lowered patient confidence in  the care received at the clinic. A low-cost yet high-tech device would be required to achieve wider adoption by clinicians. % that serve the majority of the population.
\squishend


\begin{figure}[t!]
\centering
    \includegraphics[width=.2\textwidth]{./figs/oaebud_case.jpg}
    \includegraphics[width=.2\textwidth]{./figs/oaebud_pcb.jpg}\\
    (a)\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  (b)
    \vskip -0.05in
\caption{{\bf OAEbuds hardware.} (a) The 3D-printed enclosure with pediatric and adult earbud tips. (b) OAEbud circuit board  beside penny for size comparison.}
\vskip -0.15in
\label{fig:oaebuds}
\end{figure}


We present OAEbuds, the first wireless earbud design  for low-cost hearing screening. Our hardware-software system reliably detects otoacoustic emissions using low-cost acoustic hardware, while being in the form-factor of a wireless earbud. The earbud hardware is designed to work across a wide demographic from new-borns to adults. By streaming the acoustic data via Bluetooth to a nearby smartphone, we eliminate the need for wires and pipes. Further by using the smartphone  only  for processing and not signal acquisition,  our wireless earbud design generalizes across smartphone models. Finally, compared to DIY devices, since our wireless earbuds is more integrated while being low-cost, it may help broaden the adoption of our   hearing screening tool.

%Finally, we design algorithms to detect OAEs in the presence of some background noise.

There are two key challenges in achieving this design with low-cost acoustic components. First, since speaker hardware components are bulky, it is challenging to incorporate a two-speaker design  into the form-factor of a wireless earbud. Our evaluation in~\xref{ddd} shows that a single low-cost speaker hardware introduce   nonlinearities that create inter-modulation signals which are difficult to differentiate from OAEs. Second,  when an acoustic signal is sent into an ear canal, it first gets reflected back from not only the inside of the earbud case but also the ear drum and  the walls of the ear canal before arriving at the cochlea. To accurately identify OAEs, it is important to determine when the reflections and echoes of the input stimuli end and the OAEs begin. 

We design a two-step algorithm for these challenges. 

\squishlist
\item {\bf Reflection time estimation.}  We send  a frequency modulated continuous wave (FMCW) signal as input stimuli. These signals get reflected back from the earbud case, the ear drum and the ear canal which we can capture at the earbud microphone. Since OAE signals are faint, these do not show up as part of these reflections. We then perform FMCW processing to estimate the time-delays corresponding to these reflections and determine the duration after which the power in these reflections reduce below a preset threshold. 

\item {\bf OAE signal extraction.} Instead of transmitting two tones, we send a train of wideband pulses  from the earbud speaker (Fig.~\ref{dsds}). Since the speed of sound  is  slower within the cochlea, the otoacoustic emissions from the cochlea are separated in time from the middle ear reflections of the input stimuli. To extract these OAE signals, we first remove  reflections by only considering the signals after the duration estimated in the previous step. We then synchronize the responses across consecutive wideband pulses and  then combine the signals  across multiple pulses to improve the SNR of the OAE signals and detect them using our low-cost earbud system (\xref{dsds}).
\squishend


We designed an open-source  wireless earbud hardware shown in Fig.~\ref{fig:oaebuds} that is capable of transmitting the above signals from its speaker and wirelessly streaming  the microphone audio via Bluetooth to a mobile device that performs the signal processing to extract the otoacoustic emissions.  We designed our OAEbuds hardware using open source eCAD software, outsourced fabrication and assembly (\$XX per unit), and 3D printed the enclosures in-house. The earbud is designed to support multiple eartip sizes that span new-born infants to adults. The battery in the earbud can be recharged via a USB connection within XXX~hours from a no-charge state. Our evaluation shows that on a single charge, the earbud can be used to perform XXX hearing tests, each lasting a minute each.


(Benchmark results): XXX

(Clinical study results): XXX


\vskip 0.05in\noindent{\bf Contributions.} We make the following contributions. 
\squishlist
\item We design the first wireless earbuds to achieve low-cost hearing screening by detecting otoacoustic emissions. 

\item  We describe techniques that combine FMCW signals with wideband pulses to separate reflections and echoes from OAEs while using a single low-cost speaker. 
%\item We use multi-microphone  processing  algorithms to address ambient noise, showing that contrary to popular belief, OAEs can be extracted outside of quiet  settings.

\item We perform a clinical study showing that our low-cost wireless earbuds can detect hearing loss with accuracies similar to a \$8000
FDA-cleared medical device.
\item Finally, we will make our code and hardware  open source to
help with adoption. 
\squishend

==> related.tex <==
\section{Related work}
\vskip 0.15in



\vskip 0.05in\noindent{\bf Health tracking using earphones.} Prior work has explored the use of earphones for monitoring physiological signals  for cardivascular sensing~\cite{cardiac1,headfi}, blood pressure measurements~\cite{ebp} and  respiration~\cite{respiratoryrate}. Earphones have also been used for sensing  jaw clenching~\cite{jawclenching}, teeth motion  and  voice detection~\cite{teethactivity,voiceactivity}. 
Prior work has  also explored the use of smartphone attachments for diagnosing middle ear conditions. \cite{chan2019detecting} designed a  paper cone that is attached to a smartphone and used a machine learning classifier to detect  middle ear fluid behind the ear drum. \cite{earhealth} used a smartphone-connected wired earphone attached to an external microphone  to  differentiate between   middle ear fluid, ear drum ruptures and  wax blockage. \cite{chan_justin_2022_6389337} presented a smartphone attachment to perform tympanometry where the pressure  within the ear canal is changed to assess the mobility of the ear drum. All these  wired systems however are designed for assessing the state of the middle ear and the ear drum. Hearing screening, in contrast, is primarily focused on the state of the cochlea. The Cochlea is part of the inner-ear that is behind the ear drum and is primarily responsible for converting sound waves into electrical impulses which are then interpreted by the brain.

\vskip 0.05in\noindent{\bf OAE detection.} Given the importance of OAEs for  hearing screening, there have recently been a couple of  independent  efforts to design   screening solutions using mobile devices. Prior work  \cite{heitmann2021mass,heitmann2017sound4all} created a smartphone interface for the probes from an existing commercial OAE device \cite{pathmedical}. In addition to not being wireless, this approach is still constrained by the cost of commercial OAE probes that are expensive. Further, since it is directly  connected to a smartphone it requires calibration for each smartphone model which is difficult to generalize.    Recent commercial approaches~\cite{otoscreen1,otoscreen2} have also proposed to use  bone conduction to monitor OAEs through a headband.  In addition to not being in the wireless earbud form factor, these have not been demonstrated to be low-cost.  Finally, \cite{heitmann2020designing} proposes to use a single transducer to measure OAEs. However it is primarily focused on the transducer characterization and does not build an end-to-end wireless earbud system. Further, none of these prior efforts have performed clinical studies  to evaluate  efficacy.


The closest to our work is recent work~\cite{nbme22} that uses the two speakers in a wired earphone to transmit two frequencies tones into the ear canal and uses an additional microphone that is placed next to the ear to perform new-born hearing screening. Our work differs from this prior work in four  critical ways. 1) \cite{nbme22} uses a wired earphone and external microphone that are connected to a smartphone. Since it uses the smartphone ADC, DAC and AGCs, it requires calibration for each  smartphone models, which is challenging to generalize across the smartphones used in low and middle-income countries.  2) It uses two frequency tones that are transmitted from  two different speakers and looks for inter-modulation between the tones to detect OAE. The challenge is that it is difficult to  incorporate two speakers pointing into the ear-canal in a wireless earbud form factor and hence the techniques used in the prior work can not be used for wireless earbuds. 3) The various hardware components in this prior work are attached using plastic pipes and glues which make it unreliable and difficult to scale.  4) While prior work detects background noise to discard measurements, it cannot operate with background noise. This is  important for operation in low and middle-income countries where silent environments are rare in many of the rural and urban community clinics. Our paper addresses the above limitations   and designs the first wireless earbuds for low-cost hearing loss screening. 





 Finally, high-end personalized commercial earphone products from companies like Nura Sound  use   OAE measurements to customize music for an  adult wearer~\cite{nurapatent,nura}. Our goal in this work is complementary in that we  create a low-cost and open-source  earbud system that is designed to achieve   hearing loss screening with accuracies similar to FDA-cleared devices. Further, our system is designed to  work across a diverse age range from new-born babies to adults.



\vskip 0.05in\noindent{\bf Earable platforms.} Recent years have seen the introduction of earbud platforms like eSense platform~\cite{esense1,esense2},  Clearbuds~\cite{clearbuds}  and OpenEarable~\cite{openearable}. eSense is designed for research and prototyping, while clearbuds achieves synchronization between microphones across two earbuds. Like eSense, the Clearbuds platform  does not have speakers or microphones facing the ear canal and is not designed for hearing loss screening. OpenEarable~\cite{openearable} supports an inward-facing ultrasonic microphone but does not support multiple inward-facing audible microphones that we use for reliable OAE sensing. We instead design an open-source wireless earbud platform  to reliably measure otoacoustic emissions for hearing loss screening using low-cost hardware components.



 %supports a wireless platform to achieve synchronization between microphones across two earbuds and is designed for binuaral speech enhancement for telephony applications. Like eSense, the Clearbuds platform  does not have speakers or microphones facing the ear canal and is not designed for hearing loss screening.

==> tech.tex <==
Our prior work~\cite{nbme22} proposed a \$10 DIY design for an OAE probe that can be connected to a smartphone. OAE tests require that the sound level of signals transmitted from the probe are calibrated to a specific sound level such that the sound level of the OAE can be maximized without being too loud for the patient. Additionally, calibrated sound levels allow for OAE test results to be compared across different clinics and OAE devices. Although our prior design uses a fixed probe design, the sound level of the transmitted signal still need to be calibrated for each smartphone model. This is because, every smartphone has it's own audio processing chain, DAC and AGC, which means that the same digital sound output index specified in software would result in a different sound level produced at the speaker for different smartphone models. Similar sound level calibration also needs to be performed for the microphone to find the mapping between the recorded digital value and the corresponding absolute sound level. This calibration is needed to ensure that recorded OAEs are above a predetermined sound level threshold. The need to calibrate the probe for every new smartphone model that needs to be supported makes it challenging to scale the system quickly to multiple clinics or countries.
